Light driven interactions in spatial predator-prey model with toxicant chemotaxis

We develop and analyze a spatial temporal model of light driven ecotoxicological processes, motivated by an aquatic predator-prey system of algae and \textsl{Daphnia} subject to a contaminant. Population dynamics are driven by light, which is periodic in time and varies with spatial depth. The existence and uniqueness of spatial and temporal dependent periodic solutions are shown and analytical functions of the solutions under parameter constraints are presented. We conduct Turing stability analyses of solutions with respect to perturbations of initial conditions. Given a perturbation to a periodic equilibrium state, we show the system will return to this equilibrium state as long as motility is fast enough and/or the reservoir depth is shallow enough. Analytical results assume some Dirichlet boundary conditions that match the periodic equilibrium state, however numerical simulations with more relaxed boundary conditions capture similar periodic solutions. The work sheds light onto spatially dependent population dynamics that are driven by periodic forces, such as light levels.

==> References.bbl.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/


%% Created for Angela Peace at 2020-12-10 21:32:56 -0600 


%% Saved with string encoding Unicode (UTF-8) 



@article{rana2018mechanistically,
	Author = {Rana, Md Masud and Dissanayake, Chandani and Juan, Lourdes and Long, Kevin R and Peace, Angela},
	Date-Added = {2020-12-10 21:32:50 -0600},
	Date-Modified = {2020-12-10 21:32:50 -0600},
	Journal = {Mathematical Biosciences and Engineering: MBE},
	Number = {1},
	Pages = {222--233},
	Title = {Mechanistically derived spatially heterogeneous producer-grazer model subject to stoichiometric constraints},
	Volume = {16},
	Year = {2018}}

@article{peace2016somatic,
	Author = {Peace, Angela and Poteat, Monica D and Wang, Hao},
	Date-Added = {2020-12-10 21:31:47 -0600},
	Date-Modified = {2020-12-10 21:31:47 -0600},
	Journal = {Journal of theoretical biology},
	Pages = {198--211},
	Publisher = {Elsevier},
	Title = {Somatic growth dilution of a toxicant in a predator--prey model under stoichiometric constraints},
	Volume = {407},
	Year = {2016}}

@article{yang2013computational,
	Author = {Yang, Jichen and Su, Jianzhong and Owens, Larrissa and Ibraguimov, Akif and Tang, Liping},
	Date-Added = {2020-12-10 21:30:59 -0600},
	Date-Modified = {2020-12-10 21:30:59 -0600},
	Journal = {Journal of immunological methods},
	Number = {1-2},
	Pages = {37--46},
	Publisher = {Elsevier},
	Title = {A computational model of fibroblast and macrophage spatial/temporal dynamics in foreign body reactions},
	Volume = {397},
	Year = {2013}}

@article{ibragimov2010stability,
	Author = {Ibragimov, AI and McNeal, Catherine J and Ritter, Laura Rylie and Walton, Jay R},
	Date-Added = {2020-12-10 21:29:28 -0600},
	Date-Modified = {2020-12-10 21:29:28 -0600},
	Journal = {Computational and Mathematical Methods in Medicine},
	Number = {1},
	Pages = {67--88},
	Publisher = {Taylor \& Francis},
	Title = {Stability analysis of a model of atherogenesis: an energy estimate approach II},
	Volume = {11},
	Year = {2010}}

@article{ibragimov2010stability2,
	Author = {Ibragimov, Akif and Ritter, Laura and Walton, Jay R},
	Date-Added = {2020-12-10 21:29:10 -0600},
	Date-Modified = {2020-12-10 21:30:38 -0600},
	Journal = {SIAM Journal on Applied Mathematics},
	Number = {7},
	Pages = {2150--2185},
	Publisher = {SIAM},
	Title = {Stability analysis of a reaction-diffusion system modeling atherogenesis},
	Volume = {70},
	Year = {2010}}

@article{miller2000haber,
	Author = {Miller, Frederick J and Schlosser, Paul M and Janszen, Derek B},
	Date-Added = {2020-12-02 15:43:57 -0600},
	Date-Modified = {2020-12-02 15:44:59 -0600},
	Journal = {Toxicology},
	Number = {1},
	Pages = {21--34},
	Publisher = {Elsevier},
	Title = {Haber's rule: a special case in a family of curves relating concentration and duration of exposure to a fixed level of response for a given endpoint},
	Volume = {149},
	Year = {2000}}

@book{filippov2013differential,
	Author = {Filippov, Aleksei Fedorovich},
	Date-Added = {2020-11-23 15:56:51 -0600},
	Date-Modified = {2020-11-23 15:56:51 -0600},
	Publisher = {Springer Science \& Business Media},
	Title = {Differential equations with discontinuous righthand sides: control systems},
	Volume = {18},
	Year = {2013}}

@article{hu2018hard,
	Author = {Hu, Sarah K and Connell, Paige E and Mesrop, Lisa Y and Caron, David A},
	Date-Added = {2020-09-22 11:00:27 -0500},
	Date-Modified = {2020-09-22 11:00:27 -0500},
	Journal = {Frontiers in Marine Science},
	Pages = {351},
	Publisher = {Frontiers},
	Title = {A hard day's night: Diel shifts in microbial eukaryotic activity in the North Pacific Subtropical Gyre},
	Volume = {5},
	Year = {2018}}

@article{ribalet2015light,
	Author = {Ribalet, Francois and Swalwell, Jarred and Clayton, Sophie and Jim{\'e}nez, Valeria and Sudek, Sebastian and Lin, Yajuan and Johnson, Zackary I and Worden, Alexandra Z and Armbrust, E Virginia},
	Date-Added = {2020-09-22 10:53:55 -0500},
	Date-Modified = {2020-09-22 10:53:55 -0500},
	Journal = {Proceedings of the National Academy of Sciences},
	Number = {26},
	Pages = {8008--8012},
	Publisher = {National Acad Sciences},
	Title = {Light-driven synchrony of Prochlorococcus growth and mortality in the subtropical Pacific gyre},
	Volume = {112},
	Year = {2015}}

@article{chaumot2003ecotoxicology,
	Author = {Chaumot, Arnaud and Charles, Sandrine and Flammarion, Patrick and Auger, Pierre},
	Date-Added = {2020-09-22 10:41:33 -0500},
	Date-Modified = {2020-09-22 10:41:33 -0500},
	Journal = {Environmental Toxicology and Chemistry: An International Journal},
	Number = {5},
	Pages = {958--969},
	Publisher = {Wiley Online Library},
	Title = {Ecotoxicology and spatial modeling in population dynamics: An illustration with brown trout},
	Volume = {22},
	Year = {2003}}

@book{jorgensen2013modelling,
	Author = {Jorgensen, Sven Erik},
	Date-Added = {2020-09-22 10:36:55 -0500},
	Date-Modified = {2020-09-22 10:36:55 -0500},
	Publisher = {Elsevier},
	Title = {Modelling in ecotoxicology},
	Year = {2013}}

@article{caswell1996demography,
	Author = {Caswell, Hal},
	Date-Added = {2020-09-22 10:22:18 -0500},
	Date-Modified = {2020-09-22 10:22:18 -0500},
	Journal = {Ecotoxicology: A hierarchical treatment},
	Pages = {255},
	Publisher = {CRC Press},
	Title = {Demography Meets Ecotoxicology: Untangling the Population Level},
	Volume = {2},
	Year = {1996}}

@article{huang2013model,
	Author = {Huang, Qihua and Parshotam, Laura and Wang, Hao and Bampfylde, Caroline and Lewis, Mark A},
	Date-Added = {2020-07-27 21:52:50 -0500},
	Date-Modified = {2020-07-27 21:52:50 -0500},
	Journal = {Journal of theoretical biology},
	Pages = {71--79},
	Publisher = {Elsevier},
	Title = {A model for the impact of contaminants on fish population dynamics},
	Volume = {334},
	Year = {2013}}

@techreport{huang2014development,
	Author = {Huang, Q and Wang, H and Lewis, MA},
	Date-Added = {2020-07-27 20:51:16 -0500},
	Date-Modified = {2020-07-27 20:51:16 -0500},
	Institution = {TR-59. 59 pp. http://hdl. handle. net/10402/era. 40140},
	Title = {Development of a Toxin-Mediated Predator-Prey Model Applicable to Aquatic Environments in the Athabasca Oil Sands Region. OSRIN Report No},
	Year = {2014}}

